SAGE:Specification-Aware Grammar Extraction for Automated Test Case Generation with LLMs

Grammar-based test case generation has proven effective for competitive programming problems, but generating valid and general grammars from natural language specifications remains a key challenge, especially under limited supervision. Context-Free Grammars with Counters (CCFGs) have recently been introduced as a formalism to represent such specifications with logical constraints by storing and reusing counter values during derivation. In this work, we explore the use of open-source large language models (LLMs) to induce CCFGs from specifications using a small number of labeled examples and verifiable reward-guided reinforcement learning. Our approach first fine-tunes an open-source LLM to perform specification-to-grammar translation, and further applies Group Relative Policy Optimization (GRPO) to enhance grammar validity and generality. We also examine the effectiveness of iterative feedback for open and closed-source LLMs in correcting syntactic and semantic errors in generated grammars. Experimental results show that our approach SAGE achieves stronger generalization and outperforms 17 open and closed-source LLMs in both grammar quality and test effectiveness, improving over the state-of-the-art by 15.92%p in grammar validity and 12.34%p in test effectiveness. We provide our implementation and dataset at the following anonymous repository:https://anonymous.4open.science/r/SAGE-5714

==> tables/_full_results.tex <==
\begin{table*}[t]
\centering
\caption{XXX: Full experimental results. It must not be included.}
\begin{tabularx}{\linewidth}{
lll
Yc
Yc
Yc
}
\toprule
\multirow{2}{*}{\vspace{-5pt}\bf Category} &
\multirow{2}{*}{\vspace{-5pt}\bf Model} &
\multirow{2}{*}{\vspace{-5pt}\bf Iter} &
\multicolumn{2}{c}{\bf Validity~(\%)} &
\multicolumn{2}{c}{\bf Effectiveness~(\%)} &
\multicolumn{2}{c}{\bf Generality~(\%)} \\

\cmidrule(r){4-5}
\cmidrule(r){6-7}
\cmidrule{8-9}

& & &
Element-based &
Set-based &
Element-based &
Set-based &
Element-based &
Set-based \\

\midrule

\multirow{1}{*}{Few-shot} & CCFGT5@1 & &
19.61 & 18.51 & 10.05 & 15.66 & 20.04 & 19.62 \\
& CCFGT5@5 & &
82.15 & 80.74 & 42.10 & 68.33 & 82.97 & 82.11 \\
& GPT@1 & &
67.69 & 67.03 & 31.72 & 53.67 & 60.32 & 55.92 \\
& GPT@5 & &
78.69 & 78.14 & 38.43 & 66.01 & 73.46 & 71.85 \\
& Gemini@1 & &
16.60 & 15.92 & 8.39 & 13.74 & 14.59 & 13.70 \\
& Gemini@5 & &
46.90 & 45.92 & 24.62 & 40.70 & 43.67 & 42.59 \\

\multirow{1}{*}{Iterative} & DeepSeek-R1-Distill-Qwen & 1 &
74.36 & 71.11 & 35.07 & 58.92 & 68.82 & 67.03 \\
& & 2 &
78.23 & 75.18 & 37.81 & 63.92 & 72.59 & 71.48 \\
& & 3 &
78.99 & 75.55 & 37.86 & 63.81 & 73.39 & 72.22 \\
& & 4 &
79.49 & 79.42 & 37.50 & 63.25 & 73.76 & 72.59 \\
& & 5 &
80.10 & 77.03 & 38.71 & 64.95 & 74.15 & 72.96 \\

& DeepSeek-R1-Distill-Qwen (+test cases) & 1 &
78.55 & 75.18 & 37.13 & 63.29 & 73.38 & 72.22 \\
& & 2 &
79.02 & 75.55 & 37.15 & 63.41 & 73.84 & 72.59 \\
& & 3 &
79.47 & 76.29 & 37.89 & 64.54 & 74.58 & 73.33 \\
& & 4 &
79.65 & 76.29 & 38.09 & 64.04 & 75.32 & 74.07 \\
& & 5 &
80.04 & 76.29 & 37.77 & 64.52 & 72.32 & 74.07 \\

& DeepSeek-R1 & 1 &
83.07 & 81.48 & 42.00 & 69.80 & 77.95 & 77.40 \\
& & 2 &
86.67 & 85.18 & 43.97 & 71.65 & 80.57 & 80.00 \\
& & 3 &
87.38 & 85.55 & 43.76 & 72.66 & 81.31 & 80.74 \\
& & 4 &
88.02 & 86.66 & 44.76 & 73.50 & 82.15 & 81.48 \\
& & 5 &
88.49 & 88.66 & 44.59 & 73.30 & 82.52 & 81.58 \\

& DeepSeek-V3 & 1 &
82.65 & 81.11 & 40.81 & 68.08 & 77.67 & 77.40 \\
& & 2 &
84.22 & 82.59 & 41.52 & 69.97 & 79.59 & 79.25 \\
& & 3 &
85.65 & 84.07 & 42.78 & 71.17 & 80.70 & 80.37 \\
& & 4 &
86.05 & 84.07 & 42.91 & 72.87 & 80.74 & 80.37 \\
& & 5 &
86.10 & 83.70 & 42.45 & 70.64 & 80.74 & 80.37 \\

\cmidrule{2-9}

\multirow{10}{*}{Baseline~(open)} &
Gemma2-9B & &
43.88 & 41.48 & 20.83 & 35.58 & 42.49 & 41.11 \\
& Qwen 2.0-7B & &
21.02 & 20.74 & 11.53 & 16.77 & 16.66 & 16.29 \\
& Qwen 2.5-coder-7B & &
39.47 & 37.77 & 18.52 & 31.53 & 36.26 & 35.55 \\
& Qwen 2.5-32B & &
75.67 & 71.85 & 30.16 & 60.91 & 72.34 & 71.11 \\
& LLaMA 3.1-8B & &
13.66 & 12.96 & 7.05 & 11.37 & 11.64 & 44.48 \\
& StarChat2-15B & &
- & - & - & - & - & - \\
& Mistral-Small-24B & &
15.53 & 14.44 & 8.31 & 12.88 & 12.52 & 11.85 \\
& DeepSeek-V2-Lite-Base & &
32.13 & 30.37 & 15.84 & 26.38 & 31.43 & 30.37 \\
& DeepSeek-LLama-7B & &
11.33 & 10.74 & 5.08 & 8.44 & 8.87 & 8.51 \\
& DeepSeek-R1-Distill-Qwen-32B & &
62.64 & 60.37 & 30.16 & 50.32 & 59.90 & 58.14 \\




\cmidrule{2-9}

\multirow{4}{*}{Training Method} &
DeepSeek-R1-Distill-Qwen-14B & &
- & - & - & - & - & - \\
& \quad + Supervised Fine-Tuning & &
- & - & - & - & - & - \\
& \quad + GRPO (Supervised only) & &
- & - & - & - & - & - \\
& \quad + GRPO (Unsupervised) & &
- & - & - & - & - & - \\
\midrule
Ground-truth & & & & & \\
\bottomrule
\end{tabularx}
\end{table*}

==> tables/ablation_study_testcase.tex <==
\begin{table}[htbp]
\centering
\caption{Comparison between with and without test cases (?) of DeepSeek-Qwen}
\begin{tabularx}{\linewidth}{
l
YY
YY
YY
}
\toprule
\multirow{2}{*}{\vspace{-5pt}Type} &
\multicolumn{2}{c}{Validity} &
\multicolumn{2}{c}{Effectiveness} &
\multicolumn{2}{c}{Generality} \\
\cmidrule(r){2-3}
\cmidrule(r){4-5}
\cmidrule{6-7}
&
Element & Set &
Element & Set &
Element & Set \\
\midrule
w/ test cases &
80.10 & 77.03 & 38.71 & 64.95 & 74.15 & 72.96 \\
w/o test cases &
80.04 & 76.29 & 37.77 & 64.52 & 72.32 & 74.07 \\
\bottomrule
\end{tabularx}
\end{table}

==> tables/experimental_results.tex <==
\begin{table*}[t]
\centering
\caption{Comparison of test case generation methods. Best scores will be highlighted in bold.}
\label{tab:results}
\begin{tabularx}{\linewidth}{
ll
Yc
Yc
Yc
}
\toprule
\multirow{2}{*}{\vspace{-5pt}\bf Category} &
\multirow{2}{*}{\vspace{-5pt}\bf Method} &
\multicolumn{2}{c}{\bf Validity~(\%)} &
\multicolumn{2}{c}{\bf Generality~(\%)} &
\multicolumn{2}{c}{\bf Effectiveness~(\%)} \\

\cmidrule(r){3-4}
\cmidrule(r){5-6}
\cmidrule{7-8}

& &
Set-based &
Element-based &
Set-based &
Element-based &
Set-based &
Element-based \\

\midrule

\multirow{3}{*}{CodeContests} &
Public &
- & & & \\ 

& Private &
& & & \\

& Generated &
& & & \\

\midrule

\multirow{2}{*}{Fuzzing} &
Public &
&  &  &  &  \\ 
& Private &
&  &  &  &  \\

\midrule

\multirow{4}{*}{Direct} &
ChatGPT-4 &
&  &  &  &  \\
& ChatGPT-4o &
&  &  &  &  \\
& Gemini
&  &  &  &  &  \\
& Claude-3.5 &
&  &  &  &  \\

\midrule

\multirow{5}{*}{Prompting} &
Gemini &
&  &  &  \\
& ChatGPT
&  &  &  &  \\
& Claude
& & & & \\ 
& DeepSeek-v3
& & & & & \\
& DeepSeek-r1 &
& & & & \\

\cmidrule{2-8}

& Gemma2-9B &
43.88 & 41.48 & 42.49 & 20.83 &35.58  \\

& Qwen 2.0-7B &
21.02 &  20.74&  16.66&  11.53& 16.77 \\

& Qwen 2.5-coder-7B            &   39.47&37.77  &  36.26&  18.52&31.53  \\
& Qwen 2.5-32B            & 75.67  &  71.85& 72.34 & 30.16 &60.91  \\
& LLaMA 3.1-8B          & 13.66 &  12.96 & 11.37 & 7.05 & 11.37 \\
& StarChat2-15B             &   &  &  &  &  \\
& Mistral-Small-24B             & 15.53  & 14.44 & 12.52 & 8.31 &  12.88\\
& DeepSeek-V2-Lite-Base             & 32.13  &30.37  & 31.43 &  15.84
& 26.38 \\ 
& DeepSeek-LLama-7B             & 11.33  &10.74  & 8.87 &  5.08
& 8.44 \\ 
& DeepSeek-Qwen-32B            &  74.36 & 71.11 &  68.82& 35.07  
& 58.92  \\\cmidrule{2-8}
& DeepSeek-Qwen-14B & 58.44 &57.03 &55.04 &27.68 &47.31 \\
& \quad + Supervised Fine-Tuning&  94.91&   93.33&  94.34&  49.19&  78.38  \\
& \quad + GRPO (Supervised only)  &   95.61 &   94.81&  95.69&  49.74&  79.56 \\
& \quad + GRPO (Unsupervised) & 95.17& 93.33  &  95.8&  48.52&   78.70 \\  \cmidrule{2-8}
& Ground-truth & & & & \\
\bottomrule
\end{tabularx}
\end{table*}
